Inverse and Quanto Inverse Options in a Black-Scholes World

Over 90% of exchange trading on crypto options has always been on the Deribit platform. This centralised crypto exchange only lists inverse products because they do not accept fiat currency. Currently, fiat-based traders can only make deposits in bitcoin, although they can withdraw both bitcoin and ether to their on-chain wallets. Likewise, other major crypto options platforms only list crypto--stablecoin trading pairs in so-called direct options, which are similar to the standard crypto options listed by the CME except the U.S. dollar is replaced by a stablecoin version. Until now a clear mathematical exposition of these products has been lacking. We discuss the sources of market incompleteness in direct and inverse options and compare their pricing and hedging characteristics. Then we discuss the useful applications of currency protected "quanto" direct and inverse options for fiat-based traders and describe their pricing and hedging characteristics, all in the Black-Scholes setting.

==> Quanto Crypto Options/appen.tex <==
\section*{Appendix A: Inverse and Quanto Inverse Option Prices and Greeks}

\begin{table}[h!]
			\centering
			  \renewcommand\thetable{A.1}
			\caption{Inverse and Quanto Inverse Option Prices and Greeks}
			\caption*{\footnotesize  We assume the tradable underlying price $S$ follows a GBM with volatility $\sigma$, where the drift depends on the discount rate $r$.  The inverse or quanto inverse call or put have strike $K$ and for the sake if clarity we omit the pre-defined $\Bar{X}$ for the quanto inverse case. Note that this need to be multiplied to the individual Greek. The residual time to maturity $\tau$ hold for all types and we use the notation $\omega  = \pm 1$ according as the option is a call or a put. Suppressing all time subscripts for simplicity we set  $d_1 = \ln \left(\frac{S}{K}\right)\left[\sigma \sqrt{\tau}\right]^{-1}+ ( r + \frac{1}{2}\sigma )\sqrt{\tau}$, $d_2 = d_1 - \sigma \sqrt{\tau}$ as well as $d_3 = d_2 - \sigma \sqrt{\tau} $.}
			\begin{tabular}{llllcc}
				\toprule
				Name  &    &   & & Inverse   & Quanto inverse      \\
				\midrule
				\midrule
				Price 
				& $f$ &  & 
				&  $\omega [ S \Phi(\omega d_1) - e^{-r\tau}K \Phi (\omega d_2)  ] $  
				& $\omega  e^{-r\tau}[\Phi(\omega d_2) - e^{(  \sigma^2-r)\tau }S^{-1}K \Phi(\omega d_3)] $
				\\
					[1.5em]
					
					
				Delta 
				& $\delta$ &       
				& $ \frac{\partial f}{\partial S}$ 
				& $\omega  \Phi(\omega d_1)$  
				& $ \omega e^{  (\sigma^2-2r) \tau } \frac{K}{S^2} \Phi(\omega d_3) $  
				  \\
				[1.5em]
				
				Gamma  
				& $\gamma$&       
				& $\frac{\partial^2 f}{\partial S^2}$ 
				& $ \frac{{ \phi}(d_1)}{S \sigma \sqrt{\tau}}$     
				&  $ e^{ (\sigma^2 -2r)  \tau} \frac{K}{S^3} \left[   \frac{ \phi(d_3)}{\sigma \sqrt{\tau}} -\omega2\Phi(\omega d_3) \right] $     	
				 \\
				[1.5em]
				
				Vega  
				& $\nu$ &       
				& $\frac{\partial f}{\partial \sigma}$ 
				&  $S \phi(d_1) \sqrt{\tau}$    
				&  $ e^{-r\tau} \left[ \phi(d_2) \sqrt{\tau} - \omega  e^{(\sigma^2-r) \tau} \sigma \tau \frac{2K }{S} \Phi(\omega d_3) \right] $    
				  \\
				[3em]
				
				Volga 
				& $\nu^\text{\tiny{$o$}}$  &       
				& $\frac{\partial^2 f}{\partial \sigma^2} $  
				& $   \sqrt{\tau} \phi(d_1) S \frac{d_1 d_2}{\sigma}  $    
				& $\!\begin{aligned}[t] & e^{-r\tau} \sqrt{\tau}\phi(d_2)  \frac{d_2 d_1}{\sigma} -\omega 2\frac{K}{S}\tau 	e^{\left(\sigma^2 -2r \right)\tau} \times \\
				&\left[ \Phi(\omega d_3)(1+2\sigma^2 \tau)-\sigma \phi(d_3)\left(\frac{-d_1}{\sigma}-\sqrt{\tau} \right)\right]
				\end{aligned}$
				     \\
				[5em]
				
				Vanna &  $\nu^\text{\tiny{$a$}}$ &       
				& $\frac{\partial^2 f}{\partial S\partial \sigma}$  
				& $ - \phi(d_1) \frac{d_2}{\sigma}$ 
				& $\!\begin{aligned}[t] & \qquad \omega e^{(\sigma^2-2r) \tau} \times \\
				& \frac{K}{S^2} \left[ 2 \tau \sigma\Phi(\omega d_3)  + \omega \phi(d_3) \left(\frac{-d_1}{\sigma} - \sqrt{\tau}\right) \right] 	
				 \end{aligned} $    
				        \\
				[5em]
				
				%	Rho &  $\rho$ &       &  $\frac{\partial f}{\partial r}$    &  $\omega K\tau \Phi(d_1) $     & tbd... &        \\
				%	[1.5em]
				Theta &  $\vartheta$ &       
				&    $-\frac{\partial f}{\partial \tau}$ 
				&   $\!\begin{aligned}[t] &\omega[-re^{-r\tau} K\Phi(\omega d_2) ] \\
				&- \frac{\sigma S \phi(d_1) }{2\sqrt{\tau}}\end{aligned}$
				& $\!\begin{aligned}[t] & -e^{-r\tau} \left(\frac{\phi(d_2)\sigma}{2\sqrt{\tau} } - \omega r \Phi(\omega d_2)\right)\\
				&  + \omega e^{(\sigma^2 -2r)\tau}\frac{K}{S}(\sigma^2 -2r) \Phi(\omega d_3) \end{aligned}$         \\

			\bottomrule
			\end{tabular}%
			\label{tab:Greeks}%
	\end{table}%

\clearpage

\section*{Appendix B: Derivation of the Greeks}

\begin{align*}
  d_2 &= \frac{\ln \left(\frac{S^{\$}_{_T}}{K}\right)+\left( r- \frac{1}{2}\sigma^2\right)\tau}{\sigma \sqrt{\tau}} \qquad   
   d_3 = \frac{\ln \left(\frac{S^{\$}_{_T}}{K}\right)+\left( r- \frac{3}{2}\sigma^2\right)\tau}{\sigma \sqrt{\tau}} = d_2-\sigma\sqrt{\tau}
\end{align*}




\begin{align*}
    \phi(d_2) & = \phi(-d_2)=  \frac{1}{\sqrt{2 \pi}} e^{-\frac{1}{2} d_2^2} \\
    \phi(d_3) &= \phi\left(d_2-\sigma\sqrt{\tau}\right) =\frac{1}{\sqrt{2 \pi}} e^{-\frac{1}{2} \left(d_2-\sigma\sqrt{\tau}\right)^2} =\frac{1}{\sqrt{2 \pi}} e^{-\frac{1}{2} \left(d^2_2- 2d_2\sigma\sqrt{\tau} +\sigma^2 \tau \right)}\\   
    &=\frac{1}{\sqrt{2 \pi}} e^{-\frac{1}{2} d^2_2} e^{d_2\sigma\sqrt{\tau}} e^{-\frac{1}{2}\sigma^2 \tau } =\phi(d_2) e^{\ln \left(\frac{S^{\$}_{_T}}{K}\right)+\left( r- \frac{1}{2}\sigma^2\right)\tau} e^{-\frac{1}{2}\sigma^2 \tau }\\ 
    &=\phi(d_2) \frac{S^{\$}_{_T}}{K} e^{\left( r- \sigma^2\right)\tau} 
\end{align*}

\begin{align*}
\frac{\partial d_2}{\partial F} = \frac{\partial d_3}{\partial F} = \frac{1}{F \sigma \sqrt{\tau}}
\end{align*}


\begin{align*}
\frac{\partial d_2}{\partial \sigma} = \frac{-\ln \left(\frac{S^{\$}_{_T}}{K}\right) -r\tau - \frac{1}{2}\sigma^2\tau}{\sigma^2 \sqrt{\tau}} \qquad   
  \frac{\partial d_3}{\partial \sigma} = \frac{-\ln \left(\frac{S^{\$}_{_T}}{K}\right) -r\tau - \frac{3}{2}\sigma^2\tau}{\sigma^2 \sqrt{\tau}} = \frac{\partial d_2}{\partial \sigma}-\sqrt{\tau}
\end{align*}

\begin{align*}
\frac{\partial d_2}{\partial \tau} =  \frac{-0.5\ln \left(\frac{S^{\$}_{_T}}{K}\right) +0.5r\tau - \frac{1}{4}\sigma^2\tau}{\sigma \sqrt{\tau^3}} \qquad   
  \frac{\partial d_3}{\partial \tau} =  \frac{-0.5\ln \left(\frac{S^{\$}_{_T}}{K}\right) +0.5r\tau - \frac{3}{4}\sigma^2\tau}{\sigma \sqrt{\tau^3}} = \frac{\partial d_2}{\partial \tau}-\frac{\sigma}{2\sqrt{\tau}}
\end{align*}


\begin{align*}
%\widehat{\delta} := \frac{\partial \widehat{f}}{\partial F}&=\frac{\partial}{\partial F} \left[ e^{-r\tau}\Phi(d_2)- e^{(y-r+\sigma^2) \tau}  \frac{K}{F} \Phi(d_3)\right]\\ 
{\delta} := \frac{\partial f}{\partial F}&=\frac{\partial}{\partial F} e^{-r\tau} \left[ \Phi (d_2) - e^{\left(\sigma^2-r\right) \tau } F_t ^{-1} K \Phi(d_3)\right]\\ 
&= e^{-r\tau} \left[ \frac{\partial \Phi(d_2)}{\partial d_2} \frac{\partial d_2}{\partial F} - e^{(\sigma^2-r)\tau} \left[-\frac{ K}{F^2} \Phi(d_3) + \frac{K}{F}  \frac{\partial \Phi(d_3)}{\partial d_3} \frac{\partial d_3}{\partial F}\right] \right]\\
&=  e^{-r\tau} \left[ \frac{\phi(d_2) }{F \sigma \sqrt{\tau}} - e^{(\sigma^2-r) \tau} \left[-\frac{K}{F^2} \Phi(d_3) + \frac{K}{F^2 \sigma \sqrt{\tau}}  \phi(d_3) \right] \right]\\
&=  e^{-r\tau} \left[\frac{\phi(d_2) }{F \sigma \sqrt{\tau}} + e^{(\sigma^2-r) \tau}  \frac{K}{F^2} \Phi(d_3) - e^{(\sigma^2-r)\tau}  \frac{K}{F^2 \sigma \sqrt{\tau}}  \phi(d_2-\sigma\sqrt{\tau}) \right]\\
&=  e^{-r\tau} \left[\frac{\phi(d_2) }{F \sigma \sqrt{\tau}} + e^{(\sigma^2-r) \tau}  \frac{K}{F^2} \Phi(d_3) - e^{(\sigma^2-r)\tau}  \frac{K}{F^2 \sigma \sqrt{\tau}} \phi(d_2) \frac{F}{K} e^{-(\sigma^2-r)\tau}\right]\\
&=e^{(\sigma^2 -2r)\tau} F^{-2}K \Phi(d_3)
\end{align*}


\begin{align*}
{\gamma} := \frac{\partial \delta}{\partial F}&=\frac{\partial}{\partial F} \left[ e^{(\sigma^2 -2r)\tau} F^{-2}K \Phi(d_3) \right]
%	&= e^{\sigma^2 \tau } \left[-\frac{2K}{F^2} \Phi(d_3) + \frac{K}{F^2} \frac{\phi(d_3)}{F \sigma \sqrt{\tau}})\right] \\
=e^{(\sigma^2-2r) \tau} F^{-3}K \left[ \frac{\phi(d_3)}{\sigma \sqrt{\tau}} -2\Phi(d_3) \right]
\end{align*}


\begin{align*}
\nu := \frac{\partial f}{\partial \sigma}&=\frac{\partial}{\partial \sigma}  e^{-r\tau} \left[ \Phi (d_2) - e^{\left(\sigma^2-r\right) \tau } F_t ^{-1} K \Phi(d_3)\right]\\ 
&= e^{-r\tau} \left[ \frac{\partial \Phi(d_2)}{\partial d_2} \frac{\partial d_2}{\partial \sigma} - \frac{K}{F} \left[ \frac{\partial e^{(\sigma^2-r) \tau}}{\partial \sigma} \Phi(d_3) +e^{(\sigma^2-r) \tau}  \frac{\partial \Phi(d_3)}{\partial d_3} \frac{\partial d_3}{\partial \sigma}\right] \right]\\
& =  e^{-r\tau} \left[\phi(d_2) \frac{\partial d_2}{\partial \sigma} - e^{(\sigma^2 -r)\tau} \frac{K}{F} \left[ 2 \tau \sigma  \Phi(d_3) + \phi(d_2 - \sigma \sqrt{\tau}) \left(\frac{\partial d_2}{\partial \sigma} - \sqrt{\tau}\right)  \right] \right] \\
& =  e^{-r\tau} \left[\phi(d_2) \frac{\partial d_2}{\partial \sigma} - e^{(\sigma^2 -r)\tau} \frac{K}{F} \left[ 2 \tau \sigma  \Phi(d_3) + \phi(d_2) e^{d_2 \sigma \sqrt{\tau}} e^{-\frac{\sigma^2 \tau}{2} } \left(\frac{\partial d_2}{\partial \sigma} - \sqrt{\tau}\right)  \right] \right] \\
& =  e^{-r\tau} \left[\phi(d_2) \frac{\partial d_2}{\partial \sigma} - e^{(\sigma^2 -r)\tau} \frac{K}{F} \left[ 2 \tau \sigma  \Phi(d_3) + \phi(d_2) \frac{F}{K} e^{-(\sigma^2-r)\tau} \left(\frac{\partial d_2}{\partial \sigma} - \sqrt{\tau}\right)  \right] \right] \\
& =  e^{-r\tau} \left[ \phi(d_2)\sqrt{\tau} - 2 e^{(\sigma^2-r) \tau} F^{-1}K \tau \sigma \Phi(d_3) \right]
\end{align*}

\begin{align*}
\vartheta := \frac{\partial f}{\partial \tau}&=\frac{\partial}{\partial \tau}  e^{-r\tau}\Phi (d_2) - e^{\left(\sigma^2-2r\right) \tau } F_t ^{-1} K \Phi(d_3)\\ 
&= \left[  \frac{\partial e^{-r\tau}}{\partial \tau} \Phi(d_2) + e^{-r\tau} \frac{\partial \Phi(d_2)}{\partial d_2} \frac{\partial d_2}{\partial \tau} \right] - \frac{K}{F} \left[ \frac{\partial e^{(\sigma^2-2r) \tau}}{\partial \tau} \Phi(d_3) +e^{(\sigma^2-r) \tau}  \frac{\partial \Phi(d_3)}{\partial d_3} \frac{\partial d_3}{\partial \tau}\right] \\
& = \left[-re^{-r\tau}\Phi (d_2) + e^{-r\tau} \phi(d_2)\frac{\partial d_2}{\partial \tau} \right] - \frac{K}{F} \left[\left(\sigma^2 -2r\right) \Phi (d_3) e^{(\sigma^2-2r)\tau} + e^{(\sigma^2-2r) \tau} \phi(d_3)\frac{\partial d_3}{\partial \tau}   \right] \\
&= \left[-re^{-r\tau}\Phi (d_2) + e^{-r\tau} \phi(d_2)\frac{\partial d_2}{\partial \tau} \right] - \\
& \qquad \qquad \qquad \frac{K}{F} \left[\left(\sigma^2 -2r\right) \Phi (d_3)e^{(\sigma^2-2r)\tau} + e^{(\sigma^2-2r) \tau} \phi(d_2-\sqrt{\tau})\left( \frac{\partial d_2}{\partial \tau} - \frac{\sigma}{2 \sqrt{\tau}} \right)   \right]\\
&= \left[-re^{-r\tau}\Phi (d_2) + e^{-r\tau} \phi(d_2)\frac{\partial d_2}{\partial \tau} \right] - \\
& \qquad \qquad \qquad \frac{K}{F} \left[\left(\sigma^2 -2r\right) \Phi (d_3)e^{(\sigma^2-2r)\tau} + e^{(\sigma^2-2r) \tau} \phi(d_2) \frac{S^{\$}_{_T}}{K} e^{\left( r- \sigma^2\right)\tau} \left( \frac{\partial d_2}{\partial \tau} - \frac{\sigma}{2 \sqrt{\tau}} \right)   \right]\\
&=\left[-re^{-r\tau}\Phi (d_2) + e^{-r\tau} \phi(d_2)\frac{\partial d_2}{\partial \tau} \right] -  \left(\sigma^2 -2r\right)\Phi (d_3) \frac{K}{F} e^{(\sigma^2-2r)\tau}-  e^{-r\tau} \phi(d_2) \left( \frac{\partial d_2}{\partial \tau} - \frac{\sigma}{2 \sqrt{\tau}} \right) \\
&=-re^{-r\tau}\Phi (d_2) + e^{-r\tau} \phi(d_2)\frac{\partial d_2}{\partial \tau}  -  \left(\sigma^2 -2r\right)\Phi (d_3) \frac{K}{F}e^{(\sigma^2-2r)\tau} -  e^{-r\tau} \phi(d_2) \frac{\partial d_2}{\partial \tau}  +   e^{-r\tau} \phi(d_2)\frac{\sigma}{2 \sqrt{\tau}}\\
&=-re^{-r\tau}\Phi (d_2) - e^{(\sigma^2-2r)\tau} \left(\sigma^2 -2r\right)\Phi (d_3) \frac{K}{F} +   e^{-r\tau} \phi(d_2)\frac{\sigma}{2 \sqrt{\tau}}\\
\end{align*}
\clearpage


\section*{Appendix C: Inverse and Quanto Inverse Greeks}


\begin{figure}[h!]
	\centering
	\small
	\renewcommand{\thefigure}{C.1}
	\caption{Inverse and Quanto Inverse Call Greeks I}
	\vspace{-0.3cm}
	\caption*{\footnotesize  Inverse and quanto inverse Greeks for calls as a function of the strike level $K^{^{_{\$}}}$ with fixed underlying $S^{^{_{\$}}}_{_t}$ and $\Bar{X}=S^{^{_{\$}}}_{_t}=\$25,000$, volatility $\sigma=75\%$ and different times to maturity: from 10 days (bold), 30 days (dashed) and 90 days (dotted).  The left, blue column represents the inverse Greeks, while the right, red column shows the quanto inverse Greeks.}
	\includegraphics[width=\textwidth]{Plot/Payoff/Call1.png}
	\label{fig:Greeks1Call}
\end{figure} 

\clearpage

\begin{figure}[h!]
	\centering
	\small
	\renewcommand{\thefigure}{C.2}
	\caption{Inverse and Quanto Inverse Call Greeks II}
	\vspace{-0.3cm}
	\caption*{\footnotesize  Inverse and quanto inverse Greeks for calls as a function of the strike $K$ with fixed underlying and predetermined conversion factor $S^{^{_{\$}}}_{_t}=\Bar{X}=\$25,000$, volatility $\sigma=75\%$ and different times to maturity: from 10 days (bold), 30 days (dashed) and 90 days (dotted).  The left, blue column represents the inverse Greeks, while the right, red column displays the quanto inverse Greeks.}
	\includegraphics[width=\textwidth]{Plot/Payoff/Call2.png}
	\label{fig:Greeks2Call}
\end{figure} 

\clearpage

\begin{figure}[h!]
	\centering
	\small
	\renewcommand{\thefigure}{C.3}
	\caption{Inverse and Quanto Inverse Put Greeks I }
	\vspace{-0.3cm}
	\caption*{\footnotesize  Inverse and quanto inverse Greeks for puts as a function of the strike $K$ with fixed underlying and predetermined conversion factor $S^{^{_{\$}}}_{_t}=\Bar{X}=\$25,000$, volatility $\sigma=75\%$ and different times to maturity: from 10 days (bold), 30 days (dashed) and 90 days (dotted).  The left, blue column represents the inverse Greeks, while the right, red column displays the quanto inverse Greeks.}
	\includegraphics[width=\textwidth]{Plot/Payoff/Put1.png}
	\label{fig:Greeks1Put}
\end{figure} 

\clearpage

\begin{figure}[h!]
	\centering
	\small
	\renewcommand{\thefigure}{C.4}
	\caption{Inverse and Quanto Inverse Put Greeks II }
	\vspace{-0.3cm}
	\caption*{\footnotesize   Inverse and quanto inverse Greeks for puts as a function of the strike $K$ with fixed underlying and predetermined conversion factor $S^{^{_{\$}}}_{_t}=\Bar{X}=\$25,000$, volatility $\sigma=75\%$ and different times to maturity: from 10 days (bold), 30 days (dashed) and 90 days (dotted).  The left, blue column represents the inverse Greeks, while the right, red column displays the quanto inverse Greeks.}
	\includegraphics[width=\textwidth]{Plot/Payoff/Put2.png}
	\label{fig:Greeks2Put}
\end{figure} 


%
%\section*{Appendix B: Incomplete Market Model}
%
%To fully understand the valuation and hedging of bitcoin options on Deribit, we need to consider the actual state of the cryptocurrency option market, which poses an unhedgable basis risk. This type of option pricing and hedging has been studied by a broad literature, see \cite{Rouge2000259} or \cite{Monoyios2004245}. We consider a similar probability space $\left(\Omega, \mathcal{F},\mathbb{P} \right)$ as in the standard inverse pricing vase and use the same underlying of the option. We now consider the fact that this asset itself is not traded but since the index represents a basket of varying quotes from different exchanges, we can find highly correlated assets to this basket. Let $Y^{^{_{\mathbb{B}}}}$ be this correlated and tradable instrument. We further assume that these assets are represented by:
%\begin{align}\label{eq:Incomplete_BTC_Dynamics}
%	\frac{dS^{^{_{\mathbb{B}}}}_t}{S^{^{_{\mathbb{B}}}}_t}& = \mu_{_{\mathbb{B}}}dt + \sigma_{_{\mathbb{B}}}dW_t^{^{_{\mathbb{B}}}} \\
%		\frac{dY^{^{_{\mathbb{B}}}}_t}{Y^{^{_{\mathbb{B}}}}_t}& = \mu dt + \sigma dW_t
%\end{align}
%  where  $W^{^{_{\mathbb{B}}}}$ and $W$ correlated  standard Brownian motions with  $ \langle dW^{^{_{\mathbb{B}}}}, dW \rangle = \rho dt$.  Note that $S$ and $Y$ are not perfectly correlated, i.e. $\mid \rho \mid <1$ and hence we cannot find a unique EMM for which the discounted value of $Y$ is a martingale under risk-neutral measure. We rewrite
%  $$W^{^{_{\mathbb{B}}}}_t= \rho W_t + \epsilon 	\hspace{-0.27em}\tildea{W}_t^{_{_{^{_{\mathbb{B}}}}}}, $$ 
%  where $\epsilon = \sqrt{1-\rho^2}$ with independent $	\tildea{W}_t^{^{_{\mathbb{B}}}}$ and $W_t$.
%
% We further denote by $\left\{\mathcal{G}_t\right\}_{0 \leq t \leq T}$ the filtration generated by $W_t^{^{_{\mathbb{B}}}}$. Note that this Brownian motion drives the non-traded inverse index asset.
%
%Assume there exists an equivalent measure $\mathbb{Q}$ to $\mathbb{P}$ on $\mathcal{F}$, then there exists adapted processes $m_{_T}$ and $g_{_T}$ where the Radon-Nykodym derivative is given by:
%\begin{equation}\label{eq:Incomplete_Radon_Nykodym}
%	\frac{d\mathbb{Q}}{d \mathbb{P}}= M_t, \ \text{where} \ \left\{M_t\right\}_{0 \leq t \leq T} \ \text{is a} \ \mathbb{P}-\text{martingale}
%\end{equation}
%and $M_t$ is given by:
%\begin{equation}\label{eq:Incomlete_M}
%	M_t = \exp \left[ \int_{0}^{t}  m_u dW_u + \int_{0}^{t} g_u	d \hspace{-0.27em}\tildea{W}^{_{_{^{_{\mathbb{B}}}}}}_u -  \frac{1}{2} \int_{0}^{t} m_u^2 du - \frac{1}{2} \int_{0}^{t} g^2_u du \right].
%\end{equation}
%Using the multidimensional Girsanov theorem we see that the processes $\left\{\tildea{W}_t,\hata{W}^{_{_{_{^{_{\mathbb{B}}}}}}}_t \right\}_{0 \leq t \leq T}$ defined by:
%\begin{align}
%	\begin{pmatrix}
%		\tildea{W}_t \\
%	\hata{W}^{_{_{_{^{_{\mathbb{B}}}}}}}_t 
%	\end{pmatrix} 
%	= 
%	\begin{pmatrix}
%		W_t + \int_{0}^{t} m_u du \\
%	\tildea{W}_t^{_{_{^{_{\mathbb{B}}}}}} + \int_{0}^{t } g_u du
%	\end{pmatrix} ,
%\end{align}
%is an independent Brownian motion under $\mathcal{O}$.  Further, the dynamics under  $\mathcal{O}$  are given by: 
%\begin{align}\label{eq:Incomplete_BTC_Dynamics}
%	\frac{dS^{^{_{\mathbb{B}}}}_t}{S^{^{_{\mathbb{B}}}}_t}& = \left( \mu_{\mathbb{B}} - \sigma_{\mathbb{B}} \left(\rho m_t +\epsilon g_t \right) \right) dt +  \sigma_{\mathbb{B}} dW_t \\
%	\frac{dY^{^{_{\mathbb{B}}}}_t}{Y^{^{_{\mathbb{B}}}}_t}& =  \left( \mu - \sigma m_t \right) dt +  \sigma d \hspace{-0.27em} \hata{W}_t,
%\end{align}
%where $\hata{W}_t = \rho \hspace{-0.27em}\tildea{W}_t + \epsilon \hspace{-0.27em} \hata{W}^{_{_{_{^{_{\mathbb{B}}}}}}}_t$ is a Brownian motion such that $ \langle d \hspace{-0.27em}\tildea{W}_t, d \hspace{-0.27em} \hata{W}_t\rangle = \rho dt$. For $\mathbb{Q}$ be be a local EMM, $Y_t$ needs to be a $\mathbb{Q}$-local martingale, i.e. iff:
%$$ \mu - m_t \sigma = r \quad \Rightarrow \quad m_t = m:= \frac{\mu -r}{\sigma}. $$
%Note that the EMM is uniquely defined. On the other hand $X$ is non-tradable which lets $g_{_T}$  be of any arbitrary form which results in an infinite set of possible EMM. We define this set as $\mathcal{M}$ which is in correspondence with the set of $g_t$. We further want to link the local martingale with an equivalent probability measure. Denote an equivalent measure  $ \tildea{\mathbb{P}}$ to  $\mathbb{P}$ on $\mathcal{G}$, the risk-neutral density given by:
%\begin{align}
%	\frac{d\hspace{-0.27em}\tildea{\mathbb{P}}}{d\mathbb{P}} &= \tildea{m}_t, \\
%	\tildea{M}_t &= \exp\left\{   -\int_{0}^{t} \theta_u dW^{^{_{\mathbb{B}}}}_u -\frac{1}{2} \int_{0}^{t} \theta^2_u du \right\},
%\end{align}
%where $\theta_t$ is a $\mathcal{G}_t$-adapted process. Under $\tildea{\mathbb{P}}$ we define $\hata{W}$ as:
%\begin{align}
%	\hata{W}_t &= W^{^{_{\mathbb{B}}}}_t+ \int_{0}^{t} \theta_u du
%\end{align}
%and underlying dynamics under $\tildea{\mathbb{P}}$ given by:
%\begin{align}
%	\frac{dS^{^{_{\mathbb{B}}}}_t}{S^{^{_{\mathbb{B}}}}_t} &= \left( \mu_{_{\mathbb{B}}} -\sigma_{_{\mathbb{B}}} \theta_t \right)dt +\sigma_{_{\mathbb{B}}} d \hspace{-0.27em} \hata{W}_t.
%\end{align}
%Note that the dynamics of the non-tradable inverse index are the same under $\mathbb{Q}$ and $\tildea{\mathbb{P}}$ when the integrands $m_t, g_t$ and $\theta_t$ are given as: $$ \rho m_t + \epsilon g_t = \theta_t.$$
% 
% Many arbitrage valuation models such as the BSM-model rely on the assumption that any option's claim can be  replicated by an portfolio and hence hedged perfectly. The absence of such a hedging portfolio leads to major difficulties for evaluating the option. 
% 
%In spirit of \cite{Monoyios2004245} we want to introduce a utility-based pricing where and investor or agent's risk preference is given by an exponential utility function $U(x)$: 
%$$ U(x)= - e^{-\gamma x},$$
%where $x$ denotes the wealth and $\gamma \in (0,1)$ depicts the risk aversion factor of an agent. Note that the exponential utility function provides a solution which is independent of the agents initial wealth.  The objective here is to maximise the expected utility of the wealth at maturity $T$. For this, an agent can construct a self-financing portfolio containing $\Delta_{_T}$ units of the traded asset $Y_{_T}$ and invest the remaining assets in a risk-less cash account. Further, we assume the investor shorts $n$ units of the inverse option with payoff $V_{_T}$. His wealth process $\left\{D_t\right\}_{0 \leq t \leq T}$ therefore follows:
%\begin{equation}
%dD_t = r D_tdt + \Delta_t Y_t \left(\left(\mu - r\right)dt + \sigma dW_t\right)
%\end{equation}
%we construct an optimization problem with initial endowment $D_t =d$ and non-traded inverse index value $S^{^{_{\mathbb{B}}}} =s$. The objective is to find a trading strategy $\left\{\pi_t\right\}_{0 \leq t \leq T}$ which results in:
%\begin{equation}
%	S_{\left\{n\right\}}(t,d,s)= \sup_{\pi \in \mathcal{P}} \mathbb{E}_{t,s}^{\mathbb{P}}\left[ U\left(D_{_T} +nV_{_T}) \right) \mid D_t =d, S^{^{_{\mathbb{B}}}} = s\right],
%\end{equation}
%where $\mathcal{P}$ is the set of admissible trading strategies, defined as in \cite{Monoyios2004245}. Note that we must assume a lower boundary for $nV_{_T}$, hence we cover long and short positions in put options but only long position in calls. Further, consider scenarios where the agent takes different positions in the derivatives:
%\begin{equation*}
%	n=\begin{cases}
%		-1, \quad &\text{seller} \\
%		0, \quad &\text{no investment in derivative} \\
%		1, \quad &\text{buyer}
%	\end{cases}
%\end{equation*}
%For the case $n=0$ the index dynamics does not have any influence on the wealth, hence we set $S_{\left\{0\right\}}(t,d) =  \sup_{\pi \in \mathcal{P}} \mathbb{E}_{t,s}\left[  - e^{-\lambda D_{_T}} \mid D_t=d\right] $. The other cases $n= \pm 1$ reflect a long or short position in the derivative, i.e. we can define an utility indifference buying ($p^{\text{\tiny bid}}$) and selling price ($p^{\text{\tiny ask}}$) as:
%\begin{align}
%	S_{\left\{-1\right\}} &= S(t,d + p^{\text{\tiny ask}}(t,d,s),s) \\
%	S_{\left\{1\right\}} &= S(t,d- p^{\text{\tiny bid}}(t,d,s),s).	
%\end{align}
%\cite{Monoyios2004245} introduces a solution to the optimisation problem using the Hamilton-Jacobi-Belman (HJB) equation. Using appropriate transformation and substitution as well the so-called distortion techniques he is able to show that the ask-price of a European option with payoff $V_{_T}$ is given by:
%\begin{equation}
%	p^{\text{\tiny ask}} = \frac{e^{-r\tau}}{\gamma \epsilon} \ln \left[ \mathbb{E}^0 \left[e^{\gamma \epsilon V_{_T}} \mid S^{^{_{\mathbb{B}}}} =s \right] \right],
%\end{equation} 
%where $ \mathbb{E}^0$ is the expectation under a probability measure $\mathbb{P}^0$ which is equivalent to the physical measure on $\mathcal{F}_t$ and corresponds to $\rho m_t + \epsilon g_t = \rho m$.
